SUDS: A Strategy for Unsupervised Drift Sampling

Supervised machine learning often encounters concept drift, where the data distribution changes over time, degrading model performance. Existing drift detection methods focus on identifying these shifts but often overlook the challenge of acquiring labeled data for model retraining after a shift occurs. We present the Strategy for Drift Sampling (SUDS), a novel method that selects homogeneous samples for retraining using existing drift detection algorithms, thereby enhancing model adaptability to evolving data. SUDS seamlessly integrates with current drift detection techniques. We also introduce the Harmonized Annotated Data Accuracy Metric (HADAM), a metric that evaluates classifier performance in relation to the quantity of annotated data required to achieve the stated performance, thereby taking into account the difficulty of acquiring labeled data. Our contributions are twofold: SUDS combines drift detection with strategic sampling to improve the retraining process, and HADAM provides a metric that balances classifier performance with the amount of labeled data, ensuring efficient resource utilization. Empirical results demonstrate the efficacy of SUDS in optimizing labeled data use in dynamic environments, significantly improving the performance of machine learning applications in real-world scenarios. Our code is open source and available at https://github.com/cfellicious/SUDS/

==> content/background.tex <==
\section{Background}
\label{sec:background}
A drift refers to changes in the different data and target distributions that can occur in many ways. 
In practice, a drift between a train and a test joint distribution given by $D_{train}(X, y)$ for the train one and $D_{test}(X, y)$ for the test one, is defined as follows:
\\
\begin{math} 
D_{train}(X, y) \ne D_{test}(X, y) 
\end{math}
\\
We consider a drift from a given train situation to a test situation. 
Drifts can result as much from changes in D(X) or D(y) as well as from changes in D(X|y) or D(y|X). 
The~\autoref{tab:drift-types} shows the different drift types as how most of the literature explains concept drifts such as with Moreno-Torres et al.~\cite{MorenoTorres2011}, or also Quiñonero-Candela Joaquin's book ~\cite{QuinoneroCandela2005} where the term "dataset shift" was cited for the first time. Storkey et al.~\cite{storkey2009training} acknowledge that dataset shift is a common problem in real-world applications and can lead to poor performance of machine learning models. 

From an unsupervised learning perspective, we know that a drift will cause problems for detection because the distribution of X, which is all we have, does not change. 
For the covariate drift and the prior probability drift, we consider a regression situation with X as the abscissa and y as the ordinate. As we can see, the D(X) distribution shifts to the right for the covariate drift, and the D(y) distribution shifts for the prior probability drift. 
%For the real drift, the virtual drift, and the rigorous concept drift, we consider a two-class classification problem. The horizontal and vertical axes correspond to the dimensions of the feature vector - the blue squares correspond to samples belonging to the first class and the green squares to those belonging to the second class. 
%(The dividing line corresponds to the decisive function of the classifier). 
As we can see in~\autoref{tab:drift-types}, the adaptation measures would not necessarily be the same in each case of drift. 
For example, after a covariate drift, it might be necessary to do some additional learning, 
to accustom the model to the features coming from the new distribution. 
Whereas, after a prior probability drift, it would be necessary to re-learn the model 
to restructure it. 
\begin{table}
	\centering
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{|c|c|c|c|}
	\hline
	Drift type                                                                                      & Distribution changes        & Before & After \\ \hline
	\begin{tabular}[c]{@{}c@{}}Covariate drift \\ (X -\textgreater y problems)\end{tabular}           & D(X) changes but not D(y|X) & 
	\includegraphics[, width=0.3\textwidth, height=30mm]{figures/background/beforecovariate.png}       &
	\includegraphics[width=0.3\textwidth, height=30mm]{figures/background/aftercovariate.png}	   
	\\ \hline
	\begin{tabular}[c]{@{}c@{}}Prior probability drift \\ (y -\textgreater X problems)\end{tabular} & D(y) changes but not D(X|y) & 
	\includegraphics[width=0.3\textwidth, height=30mm]{figures/background/beforepriorprob.png}       & 
	\includegraphics[width=0.3\textwidth, height=30mm]{figures/background/afterpriorprob.png}	   
	\\ \hline
	\begin{tabular}[c]{@{}c@{}}Real drift \\ (X -\textgreater y problems):\end{tabular}               & D(y|X) changes but not D(X) 
	&
	  \includegraphics[width=0.3\textwidth, height=30mm]{figures/background/background.png}  &
  
	  \includegraphics[width=0.3\textwidth, height=30mm]{figures/background/background_real_concept_drift.png}  
   \\ \hline
	\begin{tabular}[c]{@{}c@{}}Virtual drift\\ (y -\textgreater X problems)\end{tabular}            & D(X|y) changes but not D(y)
	&
	  \includegraphics[width=0.3\textwidth, height=30mm]{figures/background/background.png}  &
  
	  \includegraphics[width=0.3\textwidth, height=30mm]{figures/background/background_virtual_concept_drift.png}  
   \\ \hline
	\begin{tabular}[c]{@{}c@{}}Rigorous concept drift \\ (Both problems)\end{tabular} &  \begin{tabular}[c]{@{}c@{}}Both D(y|X) and D(X) change \\ or both D(X|y) and D(y) change\end{tabular} 
	&

	\includegraphics[width=0.3\textwidth, height=30mm]{figures/background/background.png}  &

	\includegraphics[width=0.3\textwidth, height=30mm]{figures/background/background_rigorous_concept_drift.png}  

	   \\ \hline
	\end{tabular}%
	}
	\caption{Data drift types}
	\label{tab:drift-types}
\end{table}



The drifts observed earlier can take different forms depending on the sequence of the samples that carry them. Thus, from a time \textit{t} to a time \textit{s}, which gives,
\begin{math}
    D(X_t, y_t) \ne D(X_s, y_s) 
\end{math}
 , but the in-between as a slow or fast data drift varies. 
The analysis from the sequential point of view is important in the sense that it allows the size of the manipulated data windows to be adjusted.

We can classify concept drifts into categories based on how the distribution evolves. Bayram et al.~\cite{bayram2022concept} classifies drifts as:
\begin{itemize}
    \item Sudden drift occurs when there is an abrupt change in the distribution, marking a shift from an old concept to a new concept. Sudden drift is also known as abrupt drift or immediate drift.
    \item Gradual drift occurs when the underlying distribution slowly changes over time. 
    \item Recurring drift occurs when a previously seen distribution occurs again after a time interval. "This type is similar to the gradual drift since the two concepts interchange in the system, but the main difference is the transition phase. In gradual drift, the old concept starts to phase out and is to be replaced with the new once increasingly. While in recurring drift, the old concepts reoccur after some time"~\cite{bayram2022concept}\cite{ramrez2017survey}.
\end{itemize}

==> tables/accuracy_comparison_without_partial_fit.tex <==
\begin{table}
    \centering
    \caption{Comparison of accuracy without Interleaved-test-then-train for D3 and OCDD along with respective SUDS modifications. The D3 and D3(SUDS) values are the mean over 25 runs with $\sigma$ in parentheses.}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Dataset & D3 & D3(SUDS)& OCDD & \makecell{OCDD\\(SUDS)}\\
    \hline
    Airlines & 56.50(0.07) & 56.50(0.35) & \textbf{59.21} & 56.07\\
    Chessweka & \textbf{58.02}(2.84) & 56.98(4.15) & 50.99 & 50.99 \\
    Covtype  & 46.75(0.11) & 40.17(6.17) & 56.38 & \textbf{57.86} \\
    Electricity & 57.57(0.56) & 55.54(2.25) & \textbf{76.55} & 66.12 \\
    LUdata & 53.05(1.00)& 55.37(4.03) & \textbf{81.53} & 78.86 \\
    Outdoor & 04.09(0.00) & 04.16(0.68) & \textbf{13.20} & 06.32\\
    Phishing & 52.63(0.83) & 52.57(1.83) & \textbf{87.88} & 86.15\\
    Poker & 55.84(0.12) & 50.87(0.48) & \textbf{65.07} & 55.66\\
    Rialto & 10.53(0.08) & 12.53(0.89) & \textbf{56.05} & 19.29\\
    Spam & 65.82(1.26) & 64.91(4.40) & \textbf{77.93} & 32.25\\
    Weather & 63.19(0.32) & 62.76(2.63) & \textbf{70.14} & 65.34\\
    \makecell{Interchanging\\RBF} & 15.96(0.33) & 10.71(0.88) & \textbf{93.14} & 11.84\\
    Mixed Drift & 16.29(0.29) & 15.07(0.85) & \textbf{39.60} & 11.55\\
    Moving RBF & 27.46(0.27) & 25.05(0.52) & \textbf{49.63} & 19.57\\
    \makecell{Moving\\Squares} & 34.54(0.41) & 27.73(0.38) & \textbf{89.89} & 28.52\\
    \makecell{Rotating\\Hyperplane} & 56.16(0.34) & 56.20(0.54) & \textbf{80.33} & 63.59\\
    Sea Big & 61.99(0.75) & 58.12(1.77) & \textbf{81.86} & 78.51\\
    Sea Stream & 59.29(1.41) & 58.78(2.88) & \textbf{82.21} & 76.70\\
    \makecell{Transient\\Chessboard} & \textbf{49.38}(0.33) & 16.23(1.44) & 48.54 & 26.29\\
    \hline
    \end{tabular}
    \label{tbl:accuracy_comparison_without_partial_fit}
\end{table}

==> tables/drop_in_accuracy.tex <==
\begin{table}
    \centering
    \caption{Comparison of the difference in accuracy with and without Interleaved-test-then-train for D3 and OCDD along with respective SUDS modifications. The values for D3 and D3(SUDS) are the difference of the mean accuracy over 25 runs.}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Dataset & D3 & D3(SUDS)& OCDD & \makecell{OCDD\\(SUDS)}\\
    \hline
    Airlines & 03.90 & 05.07 & 01.87 & 06.78 \\
    Chessweka & 09.96 & 10.85 & 14.23 & 14.23 \\
    Covtype  & 40.46 & 42.53 & 28.33 & 26.18\\
    Electricity & 28.94 & 25.06 & 07.14 & 13.30\\
    LUdata & 35.38 & 34.31 & 04.24 & 11.87\\
    Outdoor & 55.91 & 57.49 & 47.09 & 56.88\\
    Phishing & 33.82 & 35.47 & 02.68 & 03.63\\
    Poker & 20.24 & 20.17 & 09.55 & 16.36\\
    Rialto & 40.03 & 30.10 & 10.64 & 29.16\\
    Spam & 17.08 & 19.93 & 07.50 & 54.79\\
    Weather & 09.01 & 08.57 & 01.52 & 05.89\\
    \makecell{Interchanging\\RBF} & 72.70 & 57.22 & 03.88 & 13.86\\
    Mixed Drift & 29.10 & 29.28 & 02.04 & 27.86\\
    Moving RBF & 24.76 & 25.66 & 02.33 & 14.50\\
    \makecell{Moving\\Squares} & 42.10 & 28.23 & 06.00 & 40.20\\
    \makecell{Rotating\\Hyperplane} & 26.82 & 28.39 & 02.27 & 20.48\\
    Sea Big & 22.38 & 25.98 & 01.31 & 09.79\\
    Sea Stream & 25.25 & 25.28 & 00.95 & 10.66\\
    \makecell{Transient\\Chessboard} & 08.05 & 33.52 & 09.07 & 23.61\\
    \hline
    \end{tabular}
    \label{tbl:drop_in_accuracy}
\end{table}
